Vehicle Sequencing at Signal-Free Intersections: Analytical Performance Guarantees Based on PDMP Formulation

Signal-free intersections are a representative application of smart and connected vehicle technologies. Although extensive results have been developed for trajectory planning and autonomous driving, the formulation and evaluation of vehicle sequencing have not been well understood.In this paper, we consider theoretical guarantees of macroscopic performance (i.e., capacity and delay) of typical sequencing policies at signal-free intersections. We model intersection traffic as a piecewise-deterministic Markov process (PDMP). We analytically characterize the intersection capacity regions and provide upper bounds on travel delay under three typical policies, viz. first-in-first-out, min-switchover, and longer-queue-first. We obtain these results by constructing policy-specific Lyapunov functions and computing mean drift of the PDMP. We also validate the results via a series of micro-simulation-based experiments.

==> sections/32_multi.tex <==
\section{Multi-OD Intersections}

In this section, we extend the capacity guarantees in Theorem~\ref{thm_two} to multi-OD intersections. Specifically, we consider three typical configurations,  i.e. four ODs with turning, four ODs without turning, and general twelve ODs; see Fig.~\ref{fig:multi}. Since these configurations are more complex than two ODs, we will focus on capacity guarantees; travel delay will also be considered if insightful results are available.
%
\begin{figure}[hbt!]
    \centering
    \subfigure[Four ODs with turning.]
    {\includegraphics[width=0.2\textwidth]{images/four_turning_config.png}
    \label{fig:four_turning_config}
    }
    \subfigure[Four ODs without turning.]
    {\includegraphics[width=0.2\textwidth]{images/four_no_turning_config.png}
    \label{fig:four_no_turning_config}
    }
    \subfigure[Twelve ODs.]
    {\includegraphics[width=0.4\textwidth]{images/twelve_config.png}
    \label{fig:twelve_config}
    }
    \caption{Multi-OD intersections studied in this paper.}
    \label{fig:multi}
\end{figure}
%

By analogy with the two-OD system in Section~\ref{sec:two}, we define PDMPs for multi-OD systems as follows. Note that the notations in this subsection are self-contained. Let $\mathcal K$ be the set of traffic classes. Class-$k$ vehicles arrive as a Poisson process of rate $\lambda_k$. The service time of a vehicle consists of an inter-vehicle headway and a crossing time defined as follows. The headway is specified by a matrix $\Theta\in\mathbb R_{\ge0}^{n\times n}$, where $n$ is the number of ODs. We assume that $\theta_{i,k}\le\theta_{j,k}$ if $i$ and $k$ are from the same origin and if $j$ and $k$ are from different origins. The crossing time is a rv with $\overline R$, variance $\sigma_R^2$, and MGF $g_R(\alpha)$, all of which are assumed to be bounded.
Let $G(t)\in\mathcal G=\cup_{n=0}^\infty(\mathcal K^n\times\mathbb Z_{>0}^n)$ be the sequence of crossing, and $U(t)\in\cup_{n=0}^\infty\mathbb Z_{\ge0}^n$ be the residual service times. 
If the sequencing at time $t$ only depends on $(G(t_-),U(t_-))$, then $\{(G(t),U(t));t\ge0\}$ is an RCLL PDMP. 
Let $\mathcal K_\kappa$ be the set of ODs with the origin $\kappa$, where $\kappa\in\{W,N,E,S\}$.
We also consider the simplified state $X(t)=[X_W(t),X_N(t),X_E(t),X_S(t)]\in\mathbb R_{\ge0}^4$, where $X_\kappa(t)=\sum_{k\in\mathcal K_\kappa}\sum_{i=1}^{N_k(t)}U_{k,i}(t)$.
Again, we assume single lanes for each direction, and thus vehicles from the same origin must follow the FIFO discipline; relaxing this assumption would involve en-route over-taking and lane-changing, which we leave for future work.
We are interested in the existence of $\overline X<\infty$ such that $\overline X=\lim_{t\to\infty}(1/t)\int_{s=6}^t\|X(s)\|_1ds$ a.s., which is defined as stability of the PDMP.

The rest of this section is devoted to detailed analysis of the three configurations in Fig.~\ref{fig:multi}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Four ODs with turning}

Consider the four-OD intersection in Fig.~\ref{fig:four_turning_config} with $\mathcal K=\{WE,WS,NS,NE\}$. 
Analogous to the two-OD system, we consider three typical policies, viz. {\bf FIFO}, {\bf MS}, and {\bf LQF}.  
FIFO can be formulated with the simplified state $X(t)$ and a discrete state $Y(t)\in\mathcal H=\mathcal K\cup\{0\}$, which tracks the class of the last vehicle entering the system before time $t$; $Y(t)=0$ means that the system is empty.
MS can be formulated with the simplified state $X(t)$ and a discrete state $Z(t)\in\mathcal K$, where $Z(t)$ tracks the class of the vehicle crossing the intersection at time $t$. A major difference from two-OD MS is that, since vehicles from the same origin must follow FIFO, the MS policy actually determines whether to discharge traffic in $\mathcal K_W=\{WE,WS\}$ or $\mathcal K_N=\{NS,NE\}$ rather than the traffic in a specific class.
LQF requires tracking the full state $(G(t),U(t))$.

This configuration can be viewed as a variation of the two-OD configuration with arrival rates $\bar\lambda_W=\lambda_{WE}+\lambda_{WS}$ and $\bar\lambda_N=\lambda_{NE}+\lambda_{NS}$ and crossing times
$$
\bar\theta_{\kappa_1,\kappa_2}=\sum_{k\in\mathcal K_{\kappa_1}}\sum_{\ell\in\mathcal K_{\kappa_2}}\frac{\lambda_k\lambda_\ell}{\lambda_{\kappa_1}\lambda_{\kappa_2}}\theta_{k,\ell},
\quad \kappa_1,\kappa_2\in\{W,N\}.
$$
Let
\begin{align}
    \bar\lambda=\begin{bmatrix}
    \bar\lambda_W\\
    \bar\lambda_N
    \end{bmatrix},
    \ 
    \bar\Theta=\begin{bmatrix}
    \bar\theta_{WW} & \bar\theta_{WN}\\
    \bar\theta_{NW} & \bar\theta_{NN}
    \end{bmatrix}.
    \label{eq_lambdabar}
\end{align}
The four-OD-with-turning configuration has a strong analogy to the two-OD configuration:

\begin{theorem}
\label{thm_four1}
The capacity and delay guarantees at a four-OD intersection with turning is equivalent to those given in Theorem~\ref{thm_two} under the respective policies, with $\lambda$ and $\Theta$ in Theorem~\ref{thm_two} replaced by $\bar\lambda$ and $\bar\Theta$ defined in \eqref{eq_lambdabar}.
\end{theorem}

For numerical examples in this section, we consider
\begin{align*}
    \Theta=\left[
    \begin{array}{cccc}
        0.5 & 0.5 & 1 & 1 \\
        0.75 & 0.75 & 1.25 & 1.25 \\
        1 & 1 & 0.5 & 0.5 \\
        1.25 & 1.25 & 0.75 & 0.75
    \end{array}
    \right],
\end{align*}
which has the unit of seconds.

\emph{Proof of Theorem~\ref{thm_four1}}.
It suffices to show that $\bar\lambda$ and $\bar\Theta$ contribute to the mean drift equivalently with $\lambda$ and $\Theta$ in Theorem~\ref{thm_two}. For FIFO, consider the Lyapunov function
$$
\bar V(y,x)=\frac12\|x\|_1^2+a_y\|x\|.
$$
Over the covering $O_m=\{x\in\mathbb R_{>0}:\|x\|_2^2<m\}$, $m=1,2,\ldots$, we have
\begin{align*}
    \mathscr A_m\bar V(y,x)=\Big(-1+\sum_{k\in\mathcal K}\lambda_k(\theta_{y,k}+\overline{R}+a_k-a_y)\Big)\|x\|_1+\mbox{constant.}
\end{align*}
By Lemma~\ref{lmm_a}, there exists $\{a_y;y\in\mathcal H\}$ such that
\begin{align*}
    \sum_{k\in\mathcal K}\lambda_k(\theta_{y,k}+\overline{R}+a_k-a_y)
\le\sum_{\kappa\in\{W,N\}}\bar\lambda_\kappa\sum_{\kappa'\in\{W,N\}}\frac{\bar\lambda_\kappa'}{\|\bar\lambda\|_1}\bar\theta_{\kappa',\kappa},
\quad y\in\mathcal H,
\end{align*}
where $\bar\lambda$ and $\bar\Theta$ are defined in \eqref{eq_lambdabar}.
The rest of the proof, including the arguments associated with MS and LQF, is analogous to Theorem~\ref{thm_two}.
\hfill$\square$

Simulation results.

Experiment results.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Four OD without turning}

Consider the four-OD configuration in Fig.~\ref{fig:four_no_turning_config} with $\mathcal K=\{WE,EW,NS,SN\}$. 
Sequencing for this configuration is considerably different from (and more complex than) the two-OD one in the following aspects.
First, {FIFO} in this configuration does not have to be strict. Since opposite ODs (i.e., WE vs. EW and NS vs. SN) do not directly interfere, no FIFO constraint will be imposed between such ODs; see Fig.~\ref{}. We call this policy the {\bf relaxed FIFO} policy. We use $k\cap \ell=\emptyset$ (resp. $k\cap \ell\ne\emptyset$) to indicate that the orbits of classes $k$ and $\ell$ do not interfere (resp. do interfere); see Table~\ref{tab:interference}. 
\begin{table}[hbt]
    \centering
    \begin{tabular}{c|c c c c}
         & WE & NS & EW & SN  \\
         \hline
         WE & N/A & Yes & No & Yes \\
         NS & Yes & N/A & Yes & No \\
         EW & No & Yes & N/A & Yes \\
         SN & Yes & No & Yes & N/A 
    \end{tabular}
    \caption{Interference matrix for ODs in Fig.~\ref{fig:four_no_turning_config}. ``Yes'' (resp. ``No'') means that two ODs interfere (resp. do not interfere) with each other.}
    \label{tab:interference}
\end{table}
Second, {\bf MS} in this configuration switches the directions to discharge if both directions being discharged are cleared; see Fig.~\ref{}.
Third, LQF in this configuration will involve synchronization of sequences in four directions, which is very complicated and thus not discussed.

\begin{theorem}
\label{thm_four2}
The four-OD configuration without turning is stabilized by
\begin{enumerate}
    \item[\ref{thm_four2}.1] relaxed FIFO if and only if
    \begin{align}
        &\lambda_k\Bigg(\lambda_\ell\Big(\sum_{\substack{j=k \mbox{ or}\\j\cap k\ne\emptyset}}\frac{\lambda_j}{\sum_{i\in\mathcal K_k}\lambda_i}\theta_{j,k}+\overline{R}\Big)+\overline{R}\Bigg)\nonumber\\
        &
        +\sqrt{\sum_{\ell:\ell\cap k=\emptyset}\Big(\lambda_\ell(\sum_{\substack{j=\ell \mbox{ or}\\j\cap \ell\ne\emptyset}}\frac{\lambda_j}{\sum_{i\in\mathcal K_k}\lambda_i}\theta_{j,k}+\overline{R})\Big)^2}<1,
        \quad \forall k\in\mathcal K,
        \label{eq_fifo4wo}
    \end{align}
    
    \item[\ref{thm_four2}.2] MS if
    \begin{align}
        \lambda_k(\theta_{k,k}+\overline{R})+\sqrt{\sum_{\ell:\ell\cap k=\emptyset}\Big(\lambda_\ell(\theta_{\ell,\ell}+\overline{R})\Big)^2}<1,
        \quad \forall k\in\mathcal K.
    \end{align}
    
    % \item MD if
    % \begin{align}
    %     \lambda_k(\max_j\theta_{k,j}+\overline{R})+\sqrt{\sum_{\ell:\ell\cap k=\emptyset}\Big(\lambda_\ell(\max_j\theta_{\ell,j}+\overline{R})\Big)^2}<1,
    %     \quad \forall k\in\mathcal K.
    % \end{align}
\end{enumerate}
\end{theorem}

For numerical examples in this section, we consider
\begin{align*}
    \Theta=\left[
    \begin{array}{cccc}
        0.5 & 0.5 & 1 & 1 \\
        0.75 & 0.75 & 1.25 & 1.25 \\
        1 & 1 & 0.5 & 0.5 \\
        1.25 & 1.25 & 0.75 & 0.75
    \end{array}
    \right],
\end{align*}
which has the unit of seconds.

The proof of Theorem~\ref{thm_four2} in the FIFO case is analogous to that of Theorem~\ref{thm_two}.
The MS case is more sophisticated due to the lack of ``coupling'' between opposite ODs, which invalidates quadratic functions as in \eqref{eq_V2}. To resolve this challenge, we used a refined Lyapunov function as follows:

The root form in the above is motivated by the technique introduced in \cite{foley2001join}, which is invented for parallel queues. Specifically, this form essentially eliminates the impact of class-$k$ arrivals if $x_k=0$. The $\epsilon$ term fixes a technical gap between the Lyapunov function in \cite{foley2001join} and the peculiar behavior of our PDMP model.

\emph{Proof of Theorem~\ref{thm_four2}.1}.
Without loss of generality, suppose that $x_1>0$ and that a class-1 vehicle is crossing.
Consider the Lyapunov function
\begin{align}
    V_3(y,x)=&\frac12\Big(\sqrt{x_1^2+x_3^2+\epsilon(x_2^2+x_4^2)}+\sqrt{x_2^2+x_4^2+\epsilon(x_1^2+x_3^2)}\Big)^2\nonumber\\
    &+a_y\Big(\sqrt{x_1^2+x_3^2+\epsilon(x_2^2+x_4^2)}+\sqrt{x_2^2+x_4^2+\epsilon(x_1^2+x_3^2)}\Big),
\end{align}
where $\epsilon>0$ is a small number.
By analogy of the proof of \cite[Proposition ??]{foley2001join}, one can show that the mean drift is given by
\begin{align*}
    \mathscr LV_3=\Bigg(
    &\frac{(-1+\lambda_1(\theta_{y,1}+\overline{R}))x_1+\lambda_2(\theta_{y,2}+\overline{R})x_2+\epsilon\Big(\lambda_3(\theta_{y,3}+\overline{R})x_3+\lambda_4(\theta_{y,4}+\overline{R})x_4\Big)}{\sqrt{x_1^2+x_3^2+\epsilon(x_2^2+x_4^2)}}\\
    &+\frac{\epsilon\Big((-1+\lambda_1(\theta_{y,1}+\overline{R}))x_1+\lambda_2(\theta_{y,2}+\overline{R})x_2\Big)+\lambda_3(\theta_{y,3}+\overline{R})x_3+\lambda_4(\theta_{y,4}+\overline{R})x_4}{\sqrt{x_1^2+x_3^2+\epsilon(x_2^2+x_4^2)}}\\
    &+\sum_{y'\ne y}\lambda_{y'}(a_{y'}-a_y)+\frac{o(\|x\|_2)}{\|x\|_2}\Bigg)\Big(\sqrt{x_1^2+x_3^2+\epsilon(x_2^2+x_4^2)}+\sqrt{x_2^2+x_4^2+\epsilon(x_1^2+x_3^2)}\Big).
\end{align*}
By \eqref{eq_fifo4wo} and by Lemma~\ref{}, there exist $a_y$ such that
\begin{align*}
    (-1+\lambda_1(\theta_{y,1}+\overline{R})+)
\end{align*}
\hfill$\square$

Simulation 
and experiment results.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{General configuration}

\begin{theorem}
A twelve-OD intersection is stabilized by the relaxed FIFO policy
\end{theorem}

==> sections/50_appx.tex <==
% \appendices
\appendix


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Existence of limit \texorpdfstring{$\overline X$}{}}
\label{sec:Xbar}

In this section, we show that the limit $\overline X$ in \eqref{eq_Xbar} exists under most practical policies if $X(t)$ is bounded in the sense of \eqref{eq_zeta}.
The key is to show that the PDMP is irreducible in the sense of \cite[p.5]{meyn1993survey}.
The irreducibility argument in the discrete state space is straightforward. For the continuous state space, note that, under most practical policies, the state $x=[0,0]$ (or $u=\{0,0\}$) can be exactly attained from any initial condition in finite time with a positive probability. Hence, the PDMP is irreducible. Since the PDMP is also bounded in the sense of \eqref{eq_zeta}, the PDMP is positive by Harris \cite[Theorem 7]{meyn1993survey}, and thus the limit in \eqref{eq_Xbar} exists.





\section*{Acknowledgment}
The authors appreciate the SJTU undergraduate students that helped with this work: Qi Dai contributed to the theoretical results, Tianhao Yao, Yunqian Yao, Jingye Lin contributed to simulation, and Siyuan Lin, Yufeng Yan contributed to the experiments.

==> sections/60_bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./images/cheng}}]{Xiangchen Cheng}
is a PhD student in Control Science and Engineering at the UM Joint Institute, Shanghai Jiao Tong University (SJTU), China. He received his B.Eng. in Electrical and Computer Engineering from SJTU in 2022. He is interested in theory and application of control and optimization for smart and connected transportation systems. His research involves ideas from stochastic processes, hybrid systems, and robust control.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./images/tang}}]{Wei Tang}
is a PhD student in Control Science and Engineering at Shanghai Jiao Tong University, China. He received the B.S. degree in automation from Nanjing University of Science and Technology, in 2008 and M.S. degree in navigation guidance and control in Shanghai Academy of Space-flight Technology, China, in 2011. His research interests include cooperative driving, multi agents system, etc. He is also working on simulation and experiments of connected and autonomous vehicles.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./images/yang}}]{Ming Yang}
is Professor at the Department of Automation, and Acting Dean of the UM Joint Institute, Shanghai Jiao Tong University (SJTU), China. He received his BS degree from Huazhong University of Science and Technology in 1997, and MS and Ph.D. degrees from Tsinghua University, China, in 1999 and 2003, respectively. He is the
Deputy Director of SJTU's Innovation Center of Intelligent Connected Vehicles, and was the Head of the Department of Automation, SJTU. He participated in several related research projects, such as the THMR-V project (first intelligent vehicle in China), European CyberCars and CyberMove projects, CyberC3 project, CyberCars-2 project, and ITER transfer cask project, AGV. He is also the recipient of numerous domestic and international awards for both research and teaching.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./images/Fig_Jin}}]{Li Jin}
is John Wu \& Jane Sun Associate Professor (2022--present) and was Assistant Professor (2021-2022) of Electrical and Computer Engineering at the UM Joint Institute and the Department of Automation, Shanghai Jiao Tong University (SJTU), China. He was Assistant Professor (2018--2020) at the Tandon School of Engineering, New York University, USA. He received his B.Eng. from SJTU in 2011, M.S. from Purdue University, USA in 2012, and Ph.D. from the Massachusetts Institute of Technology, USA in 2018. He was also a Visiting Scholar at the University of Erlangen-Nuremberg, Germany in 2016. He is the recipient of multiple research grants/awards from the US National Science Foundation and the National Natural Science Foundation of China on topics including highway traffic control, connected and autonomous vehicles, and cyber-physical security.
\end{IEEEbiography}
